If It's Not Enough, Make It So: Reducing Authentic Data Demand in Face Recognition through Synthetic Faces

Recent advances in deep face recognition have spurred a growing demand for large, diverse, and manually annotated face datasets. Acquiring authentic, high-quality data for face recognition has proven to be a challenge, primarily due to privacy concerns. Large face datasets are primarily sourced from web-based images, lacking explicit user consent. In this paper, we examine whether and how synthetic face data can be used to train effective face recognition models with reduced reliance on authentic images, thereby mitigating data collection concerns. First, we explored the performance gap among recent state-of-the-art face recognition models, trained with synthetic data only and authentic (scarce) data only. Then, we deepened our analysis by training a state-of-the-art backbone with various combinations of synthetic and authentic data, gaining insights into optimizing the limited use of the latter for verification accuracy. Finally, we assessed the effectiveness of data augmentation approaches on synthetic and authentic data, with the same goal in mind. Our results highlighted the effectiveness of FR trained on combined datasets, particularly when combined with appropriate augmentation techniques.

==> RQ1.tex <==
\begin{table*}[t]
\begin{center}
\resizebox{.5\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline Train Data & Id/Img. & LFW $(\uparrow)$ & AgeDB-30 $(\uparrow)$ & CFP-FP $(\uparrow)$ & CA-LFW $(\uparrow)$ & CP-LFW $(\uparrow)$ & Avg $(\uparrow)$ \\
\hline GC & $10 \mathrm{~K} / 50$ & 93.22 & 77.60 & 73.03 & 82.25 & 70.80 & 79.38 \\
\hline DC & $10 \mathrm{~K} / 50$ & 98.55 & 89.70 & 85.33 & 91.60 & 82.62 & 89.56 \\
\hline \hline WF (1K) & $1 \mathrm{~K} / 45$ & 95.60 & 81.97 & 80.81 & 84.78 & 76.83 &  83.99 \\
\hline WF (2K) & $2 \mathrm{~K} / 45$ & 97.23 & 86.30 & 87.88 & 89.36 & 82.07 & 88.57 \\
\hline WF (4K) & $4 \mathrm{~K} / 45$ & 97.76 & 91.32 & 91.70 & 91.72 & 85.98 & 91.69 \\
\hline WF (6K) & $6 \mathrm{~K} / 46$ & 99.25 & 93.80 & 93.36 & 92.85 & 88.77 & 93.61 \\
\hline WF (8K) & $8 \mathrm{~K} / 46$ & 99.35 & 94.71 & 95.01 & 93.18 & 89.25 & 93.90 \\
\hline WF (10K) & $10 \mathrm{~K} / 46$ & \color{blue}{\textbf{99.55}} & 94.55 & 95.31 & 93.78 & 89.95 & 94.63 \\
%[91.49, 93.13, 93.52, 94.55, 94.73, 93.02, 94.27, 94.41, 95.08, nan]
\hline \hline GC (10K) $\cup$ WF (1K) & $11 \mathrm{~K} / 49$ & 97.95 & 88.80 & 87.24 & 89.68 & 83.57 & 89.44 \\
\hline GC (10K) $\cup$ WF (2K) & $12 \mathrm{~K} / 49$ & \textbf{98.67} & \textbf{90.45} & \textbf{90.90} & \textbf{91.50} & \textbf{85.92} & \textbf{91.49}  \\ 
\hline GC (10K) $\cup$ WF (4K) & $14 \mathrm{~K} / 49$ & 99.27 & 92.57 & 93.06 & 92.32 & 88.45 & 93.13 \\
\hline GC (10K) $\cup$ WF (6K) & $16 \mathrm{~K} / 49$ & \textbf{99.38} & 93.30 & \textbf{94.39} & 91.12 & \textbf{89.43} & 93.52 \\
\hline GC (10K) $\cup$ WF (8K) & $18 \mathrm{~K} / 48$ & 99.46 & 94.23 & 95.23 & 93.37 & 90.47 & 94.55 \\
\hline GC (10K) $\cup$ WF (10K) & $20 \mathrm{~K} / 48$ & 99.52 & 94.53 & 95.26 & \textbf{93.82} & \textbf{90.53} & \textbf{94.73} \\

\hline \hline DC (10K) $\cup$ WF (1K) & $11 \mathrm{~K} / 49$ & 99.13 & 93.45 & 92.83 & 92.43 & 87.63 & 93.09 \\
\hline DC (10K) $\cup$ WF (2K) & $12 \mathrm{~K} / 49$ & \textbf{99.15} & \textbf{93.03} & \textbf{92.61} & \textbf{92.52} & \textbf{87.78} & \textbf{93.02}  \\ 
\hline DC (10K) $\cup$ WF (4K) & $14 \mathrm{~K} / 49$ & 99.45 & 94.47 & 94.64 & 93.20 & 89.58 & 94.27 \\
\hline DC (10K) $\cup$ WF (6K) & $16 \mathrm{~K} / 49$ & \textbf{99.42} & \textbf{94.35} & \textbf{94.59} & \textbf{93.73} & \textbf{89.97} & \textbf{94.41} \\
\hline DC (10K) $\cup$ WF (8K) & $18 \mathrm{~K} / 49$ & 99.55 & 95.15 & 95.88 & 93.83 & 90.98 &  95.08 \\
\hline DC (10K) $\cup$ WF (10K) & $20 \mathrm{~K} / 49$ & 99.50 & \color{blue}{\textbf{94.92}} & \color{blue}{\textbf{95.71}} & \color{blue}{\textbf{94.08}} & \color{blue}{\textbf{90.98}} & \color{blue}{\textbf{95.06}} \\
%\hline \hline GC (1K) (10K) $\cup$ WF (9K)  & $10 \mathrm{~K} / 46$ & 99.43 & 94.62 & 95.10 & 93.12 & 90.02 & 94.46  \\
%\hline GC (2K) (10K) $\cup$ WF (8K) & $10 \mathrm{~K} / 47$ & 99.35 & 94.07 & 95.19 & 93.05 & 89.78 & 94.29  \\
%\hline GC (3K) (10K) $\cup$ WF (7K) & $10 \mathrm{~K} / 47$ & 99.35 & 93.58 & 94.90 & 92.98 & 89.73 & 94.11  \\
%\hline GC (4K) (10K) $\cup$ WF (6K) & $10 \mathrm{~K} / 48$ & 99.38 & 93.68 & 94.10 & 92.67 & 89.43 & 93.85  \\
%\hline GC (5K) (10K) $\cup$ WF (5K) & $10 \mathrm{~K} / 48$ & 99.30 & 93.42 & 93.34 & 92.60 & 89.07 & 93.55  \\
%\hline GC (6K) (10K) $\cup$ WF (4K) & $10 \mathrm{~K} / 48$ & 99.17 & 92.18 & 92.87 & 92.45 & 88.05 & 92.94  \\
%\hline GC (7K) (10K) $\cup$ WF (3K) & $10 \mathrm{~K} / 49$ & 98.93 & 91.93 & 91.97 & 91.82 & 86.98 & 92.33  \\
%\hline GC (8K) (10K) $\cup$ WF (2K) & $10 \mathrm{~K} / 49$ & 98.62 & 90.18 & 89.60 & 90.45 & 85.68 & 90.91  \\
%\hline GC (9K) (10K) $\cup$ WF (1K) & $10 \mathrm{~K} / 50$ & 98.17 & 89.15 & 87.49 & 88.78 & 83.30 & 89.38  \\

%\hline \hline DC (1K) (10K) $\cup$ WF (9K)  & $10 \mathrm{~K} / 46$ & 99.50 & 94.38 & 95.43 & 93.63 & 90.10 & 94.61 \\
%\hline DC (2K) (10K) $\cup$ WF (8K) & $10 \mathrm{~K} / 47$ & 99.45 & 94.65 & 95.56 & 93.55 & 90.18 & 94.68 \\
%\hline DC (3K) (10K) $\cup$ WF (7K) & $10 \mathrm{~K} / 47$ & 99.33 & 94.75 & 95.14 & 93.52 & 90.13 & 94,57 \\
%\hline DC (4K) (10K) $\cup$ WF (6K) & $10 \mathrm{~K} / 48$ & 99.43 & 94.28 & 95.01 & 93.42 & 90.45 & 94.52 \\
%\hline DC (5K) (10K) $\cup$ WF (5K) & $10 \mathrm{~K} / 48$ & 99.37 & 94.25 & 94.90 & 93.33 & 89.57 & 94.28 \\
%\hline DC (6K) (10K) $\cup$ WF (4K) & $10 \mathrm{~K} / 48$ & 99.27 & 94.10 & 94.41 & 93.33 & 89.52 & 94.13 \\
%\hline DC (7K) (10K) $\cup$ WF (3K) & $10 \mathrm{~K} / 49$ & 99.35 & 93.55 & 94.27 & 92.87 & 89.03 & 93.81 \\
%\hline DC (8K) (10K) $\cup$ WF (2K) & $10 \mathrm{~K} / 49$ & 99.17 & 93.27 & 93.77 & 92.68 & 88.10 & 93.40 \\
%\hline DC (9K) (10K) $\cup$ WF (1K) & $10 \mathrm{~K} / 50$ & 99.03 & 93.20 & 92.54 & 92.23 & 87.32 & 92.86 \\
\hline
\end{tabular}
}

    
\end{center}
\vspace{1mm}
\caption{Verification accuracy comparison between real-data, synthetic data and mixed-domain-data performances on five benchmark datasets (the higher, the better). Absolute best accuracies in {\color{blue}{\textbf{blue}}}. In the last six rows, results in \textbf{bold} highlight performances better than the two baselines (the corresponding synthetic one and the real one with the same amount of real identities). GC stands for GC, while WF stands for CASIA-WF.}

\label{table:RQ1}
\end{table*}

==> RQ1_sup.tex <==
\begin{subtable}{.95\linewidth}{
\begin{center}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline Train Data & Id/Img. & LFW $(\uparrow)$ & AgeDB-30 $(\uparrow)$ & CFP-FP $(\uparrow)$ & CA-LFW $(\uparrow)$ & CP-LFW $(\uparrow)$ & Avg $(\uparrow)$ \\
\hline
\hline GC & $10 \mathrm{~K} / 50$ & 93.22 & 77.60 & 73.03 & 82.25 & 70.80 & 79.38 \\
\hline DC & $10 \mathrm{~K} / 50$ & 98.55 & 89.70 & 85.33 & 91.60 & 82.62 & 89.56 \\
\hline
\end{tabular}
}  
\end{center}}
\vspace{-3mm}
\caption{Synthetic baselines verification accuracy.}
\label{table:RQ1sup}
\end{subtable}

==> RQ1b.tex <==
\begin{table}[t]
\begin{center}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline Train Data & Id/Img. & LFW $(\uparrow)$ & AgeDB-30 $(\uparrow)$ & CFP-FP $(\uparrow)$ & CA-LFW $(\uparrow)$ & CP-LFW $(\uparrow)$ & Avg $(\uparrow)$ \\
\hline
\hline GC (10K) & 10K / 50 & 93.22 & 77.60 & 73.03 & 82.25 & 70.80 & 79.38 \\
\hline DC (10K) & 10K / 50 & \textbf{98.55} & \textbf{89.70} & \textbf{85.33} & \textbf{91.60} & \textbf{82.62} & \textbf{89.56} \\
\hline WF (10K) & 10K / 46 & \textbf{94.55} & 99.55  & \textbf{95.31} & \textbf{93.78} & \textbf{89.95} & \textbf{94.63} \\ 
\hline
\end{tabular}
}   
\end{center}
\vspace{-2mm}
\caption{Verification accuracies in \% on five different benchmarks, presenting the ones achieved by the models trained on synthetic GC and DC datasets and on the . The second group of results presented the achieved performance using different subsets of authentic WF. The last two groups of results presented the achieved verification accuracies by combining different subsets of authentic WF with synthetic GC and DC datasets. It can be clearly noticed that the performances of synthetic-based FR models improved by adding a limited subset of authentic data. 
%(the higher, the better) across combined training data ratios with a fixed total number of identities (10K).  
Best accuracy for each benchmark in \textbf{bold}.}

\label{table:RQ1b}
\end{table}

==> RQ2dc.tex <==
\begin{table}[h]
\begin{center}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline Train Data & Method & LFW $(\uparrow)$ & AgeDB-30 $(\uparrow)$ & CFP-FP $(\uparrow)$ & CA-LFW $(\uparrow)$ & CP-LFW $(\uparrow)$ & Avg $(\uparrow)$ \\
\hline DC (10K) $\cup$ WF (1K) & - & 99.13 &  93.45 &  92.83 &  92.43 & 87.63 &  \textbf{93.09}  \\ 
\hline DC (10K) $\cup$ WF (1K) & MixStyle &  99.15 & 92.88 & 92.01 & 92.13 &  86.95 & 92.62   \\
\hline 
\hline DC (10K) $\cup$ WF (2K) & - &  99.15 &  93.03 &  92.61 & 92.52 &  87.78 &  \textbf{93.02}  \\ 
\hline DC (10K) $\cup$ WF (2K) & MixStyle & 99.08 & 92.83 & 92.34 &  92.63 & 87.73 & 92.85 \\
\hline 
\hline DC (10K) $\cup$ WF (4K) & - & 99.45 &  94.47 &  94.64 & 93.20 &  89.58 &  \textbf{94.27}   \\ 
\hline DC (10K) $\cup$ WF (4K) & MixStyle & 99.45 & 93.78 & 94.33 &  93.50 & 88.58 & 93.93 \\
\hline 
\hline DC (10K) $\cup$ WF (6K) & - &  99.42	& 94.35	& 94.59	&  93.73	&  89.97	&  \textbf{94.41} \\
\hline DC (10K) $\cup$ WF (6K) & MixStyle & 99.40	&  94.36	&  94.87	& 93.28	& 89.58	& 94.30 \\
\hline 
\hline DC (10K) $\cup$ WF (8K) & - &  99.55 &  95.15 &  95.88 & 93.83 &  90.98 &   \textbf{95.08}   \\ 
\hline DC (10K) $\cup$ WF (8K) & MixStyle & 99.52 & 94.68 & 95.19 &  93.97 & 89.90 & 94.65 \\
\hline 
\hline DC (10K) $\cup$ WF (10K) & -&  99.50	& 94.92	&  95.71	&  94.08	&  90.98	&  \textbf{95.04} \\
\hline DC (10K) $\cup$ WF (10K) & MixStyle & 99.47 &  95.17 & 95.58 & 93.95 & 89.97 & 94.83 \\
\hline
\end{tabular}}
\end{center}
\vspace{-1mm}
\caption{Impact of the application of the MixStyle domain generalization method on the training dataset on FR verification accuracies. We report the comparison for different subsets of the authentic dataset combined with the synthetic dataset
For each group of experimental settings, the best average accuracy is in \textbf{bold}.
The authentic identities are sampled from WF and the synthetic ones are from DC.}
\vspace{1mm}
\label{table:RQ2-dc}
\end{table}

==> RQ2gc.tex <==
\begin{table}[h]
\begin{center}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline Train Data & Method & LFW $(\uparrow)$ & AgeDB-30 $(\uparrow)$ & CFP-FP $(\uparrow)$ & CA-LFW $(\uparrow)$ & CP-LFW $(\uparrow)$ & Avg $(\uparrow)$ \\
\hline GC (10K) $\cup$ WF (1K) & - &  97.95 &  88.80 & 87.24 & 89.68 &  83.57 &  \textbf{89.44}  \\ 
\hline GC (10K) $\cup$ WF (1K) & MixStyle & 97.93 & 87.48 &  88.07 &  89.80 & 82.53 & 89.16 \\
\hline 
\hline GC (10K) $\cup$ WF (2K) & - & 98.67 &  90.45 &  90.90 &  91.50 &  85.92 &  \textbf{91.49}  \\ 
\hline GC (10K) $\cup$ WF (2K) & MixStyle & 98.67 & 90.08 & 90.53 & 91.00 & 85.70 & 91.20 \\
\hline 
\hline GC (10K) $\cup$ WF (4K) & -        &  99.27 &  92.57 &  93.06 & 92.32 &  88.45 &  \textbf{93.13} \\ 
\hline GC (10K) $\cup$ WF (4K) & MixStyle & 99.17 & 91.87 & 92.88 &  92.78 & 88.18 & 92.98 \\
\hline 
\hline GC (10K) $\cup$ WF (6K) & - &  99.38 &  93.30 &  94.39 & 91.12 &  89.43 &  \textbf{93.52} \\
\hline GC (10K) $\cup$ WF (6K) & MixStyle & 99.33 & 92.33 & 93.93 &  92.40 & 89.08 & 93.41 \\
\hline 
\hline GC (10K) $\cup$ WF (8K) & -        & 99.46 &  94.23 &  95.23 & 93.37 &  90.47 &  \textbf{94.55}  \\ 
\hline GC (10K) $\cup$ WF (8K) & MixStyle &  99.48 & 93.78 & 94.86 &  93.53 & 90.07 & 94.34 \\
\hline 
\hline GC (10K) $\cup$ WF (10K) & - & 99.52 &  94.53 &  95.26 &  93.82 &  90.53 &  \textbf{94.73} \\
\hline GC (10K) $\cup$ WF (10K) & MixStyle &  99.55 & 94.00 & 95.23 & 93.47 & 90.15 & 94.48 \\
\hline
\end{tabular}}
\end{center}
\vspace{-1mm}
\caption{Impact of the application of the MixStyle domain generalization method on the training dataset on FR verification accuracies. We report the comparison for different subsets of the authentic dataset combined with the synthetic dataset
For each group of experimental settings, the best average accuracy is in \textbf{bold}.
The authentic identities are sampled from WF and the synthetic ones are from GC.}
\vspace{1mm}
\label{table:RQ2-gc}
\end{table}


==> RQ3dc.tex <==
\begin{table*}[t!]
\begin{center}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline Train Data & Method & LFW $(\uparrow)$ & AgeDB-30 $(\uparrow)$ & CFP-FP $(\uparrow)$ & CA-LFW $(\uparrow)$ & CP-LFW $(\uparrow)$ & Avg $(\uparrow)$ \\
\hline DC (10K) $\cup$ WF (1K) & - &  99.13 &  93.45 &  92.83 &  92.43 &  87.63 &  \textbf{93.09}  \\ 
\hline DC (10K) $\cup$ WF (1K) & Sampling & 99.05 & 91.63 & 91.94 & 91.65 & 85.67 & 91.99 \\
\hline 
\hline DC (10K) $\cup$ WF (2K) & - &  99.15 &  93.03 & 92.61 &  92.52 &  87.78 &  \textbf{93.02}  \\ 
\hline DC (10K) $\cup$ WF (2K) & Sampling & 99.13 & 92.28 &  92.67 & 91.98 & 86.32 & 92.48 \\
\hline 
\hline DC (10K) $\cup$ WF (4K) & - &  99.45 &  94.47 &  94.64 &  93.20 &  89.58 &  \textbf{94.27}   \\ 
\hline DC (10K) $\cup$ WF (4K) & Sampling & 99.25 & 93.67 & 94.17 & 92.73 & 88.35 & 93.63 \\
\hline 
\hline DC (10K) $\cup$ WF (6K) & - &  99.42	&  94.35	& 94.59	&  93.73	&  89.97	&  \textbf{94.41} \\
\hline DC (10K) $\cup$ WF (6K) & Sampling & 99.25	& 93.83	&  95.03	& 93.22	& 89.02 & 94.07 \\
\hline 
\hline DC (10K) $\cup$ WF (8K) & - &  99.55 &  95.15 &  95.88 & 93.83 &  90.98 &   \textbf{95.08}   \\ 
\hline DC (10K) $\cup$ WF (8K) & Sampling & 99.48 & 94.52 & 95.46 &  93.88 & 89.68 & 94.60\\
\hline 
\end{tabular}}
\end{center}
\vspace{-1mm}
\caption{Impact of authentic identities utility-based sampling on FR verification accuracies. We report the comparison for different subsets of the authentic dataset combined with the synthetic dataset
For each group of experimental settings, the best average accuracy is in \textbf{bold}.
The authentic identities are sampled from WF and the synthetic ones are from DC.}
\vspace{1mm}
\label{table:RQ3dc}
\end{table*}

==> RQ3gc.tex <==
\begin{table}[h]
\begin{center}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline Train Data & Method & LFW $(\uparrow)$ & AgeDB-30 $(\uparrow)$ & CFP-FP $(\uparrow)$ & CA-LFW $(\uparrow)$ & CP-LFW $(\uparrow)$ & Avg $(\uparrow)$ \\
\hline GC (10K) $\cup$ WF (1K) & - & 97.95 &  88.80 &  87.24 &  89.68 &  83.57 &  \textbf{89.44}  \\ 
\hline GC (10K) $\cup$ WF (1K) & Sampling & 97.95 & 85.90 & 86.19 & 87.62 & 80.28 & 87.59  \\
\hline 
\hline GC (10K) $\cup$ WF (2K) & -& 98.67 &  90.45 &  90.90 &  91.50 &  85.92 &  \textbf{91.49}  \\ 
\hline GC (10K) $\cup$ WF (2K) & Sampling &  98.78 & 90.17 & 90.21 & 91.33 & 85.30 & 91.16 \\
\hline 
\hline GC (10K) $\cup$ WF (4K) & - &  99.27 &  92.57 & 93.06 &  92.32 &  88.45 &  \textbf{93.13} \\ 
\hline GC (10K) $\cup$ WF (4K) & Sampling & 99.07 & 91.52 &  93.21 & 92.30 & 87.62 & 92.74 \\
\hline 
\hline GC (10K) $\cup$ WF (6K) & - &  99.38 & 93.30 & 94.39 & 91.12 &  89.43 & 93.52 \\
\hline GC (10K) $\cup$ WF (6K) & Sampling & 99.30 &  93.42 &  94.46 &  93.25 & 89.41 &  \textbf{93.97} \\
\hline 
\hline GC (10K) $\cup$ WF (8K) & - &  99.46 &  94.23 &  95.23 & 93.37 &  90.47 &  \textbf{94.55} \\ 
\hline GC (10K) $\cup$ WF (8K) & Sampling & 99.42 & 94.03 & 95.13 &  93.53 & 90.05 & 94.43 \\
\hline

\end{tabular}}
\end{center}
\vspace{-1mm}
\caption{Impact of authentic identities utility-based sampling on FR verification accuracies. We report the comparison for different subsets of the authentic dataset combined with the synthetic dataset
For each group of experimental settings, the best average accuracy is in \textbf{bold}.
The authentic identities are sampled from WF and the synthetic ones are from DC.}
\vspace{1mm}
\label{table:RQ3gc}
\end{table}
